Unsupervised Machine Learning for Explainable Health Care Fraud Detection

The US federal government spends more than a trillion dollars per year on health care, largely provided by private third parties and reimbursed by the government. A major concern in this system is overbilling, waste and fraud by providers, who face incentives to misreport on their claims in order to receive higher payments. In this paper, we develop novel machine learning tools to identify providers that overbill Medicare, the US federal health insurance program for elderly adults and the disabled. Using large-scale Medicare claims data, we identify patterns consistent with fraud or overbilling among inpatient hospitalizations. Our proposed approach for Medicare fraud detection is fully unsupervised, not relying on any labeled training data, and is explainable to end users, providing reasoning and interpretable insights into the potentially suspicious behavior of the flagged providers. Data from the Department of Justice on providers facing anti-fraud lawsuits and several case studies validate our approach and findings both quantitatively and qualitatively.

==> 040results.tex <==
Descriptive on driving factors
\begin{enumerate}
    \item Which ICD9 codes drive overbilling?
    \item Where do they live in medicine? What do they mean, what are they related to?
    \item Sensitivity to types of fraud
    \item When a hospital gets picked out by DOJ, what was it for?
    \item Which types of caught hospitals are we catching?
    \item Combine this with our shap ICD9 codes; are we finding the same ICD9 codes as the DOJ?
    \begin{itemize}
        \item No positive results found yet
    \end{itemize}
    \item Linguistic similar between ICD9 description and the DOJ press release 
\end{enumerate}











